Acoustical Analysis of Speech Under Physical Stress in Relation to Physical Activities and Physical Literacy

Human speech production encompasses physiological processes that naturally react to physic stress. Stress caused by physical activity (PA), e.g., running, may lead to significant changes in a person's speech. The major changes are related to the aspects of pitch level, speaking rate, pause pattern, and breathiness. The extent of change depends presumably on physical fitness and well-being of the person, as well as intensity of PA. The general wellness of a person is further related to his/her physical literacy (PL), which refers to a holistic description of engagement in PA. This paper presents the development of a Cantonese speech database that contains audio recordings of speech before and after physical exercises of different intensity levels. The corpus design and data collection process are described. Preliminary results of acoustical analysis are presented to illustrate the impact of PA on pitch level, pitch range, speaking and articulation rate, and time duration of pauses. It is also noted that the effect of PA is correlated to some of the PA and PL measures.

==> draft.tex <==
\section{Acoustic Phone Embedding}\label{embed}

    \subsection{Recurrent autoencoder (RAE)}
The encoder-decoder based RAE is an unsupervised neural network model. One common application of RAE is to extract the compact representations from variable length sequences, e.g. Chung at el. \cite{chung2016audio} demonstrated the use of RAE to map unlabelled speech segment into fixed dimensional representation in spoken term detection (STD) task. % Yet to be edited...Kamper \cite{kamper2019truly} 
The RAE operates in three stages. The encoder first receives the input sequence. The hidden state of the encoder's last layer then reaches the linear layer and generates the embedding, which is fed into the decoder to construct the output sequence. 
Each embeddings is desired to reconstruct its input sequence through the decoder. %In this sense the embedding is expected to compactly
%In One goal of the RAE is to generate an embedding $\boldsymbol{z}$ such that the decoder output is closest to the encoder input in the Euclidean space. 
This can achieved by using the mean squared error (MSE) loss in the training stage. For each input speech segment $S = [\: \boldsymbol{x_{1}, x_{2}, x_{3},...,x_{T}}\:]$, the MSE loss is

\begin{equation} \label{MSE}
L_{mse}=\sum_{t=1}^{T} \| \boldsymbol{x_{t}} - D_{t}(E(S)) \| ^2    
\end{equation}
where $D_{t}(\cdot)$ refers to the decoder output at time step $t$ and $E(\cdot)$ denotes the last hidden layer output of the encoder, while $T$ represents the segment length.
In this work we adopt the gated recurrent units (GRU). It is a branch of recurrent neural network (RNN). GRU has simpler network structure than long short term memory network (LSTM) which speeds up the training. The implementation can be referred to \cite{audhkhasi2017end}.

    \subsection{Correspondence Recurrent Autoencoder (Cor-RAE)}
Contrary to standard RAE, the Cor-RAE weakens the input-output constraint which no longer enforces identical input-output sequence in model training. As an alternative, the input-output pair in Cor-RAE training are separately drawn from different instances of the same class. In our work, the class refers to phone category.
The loose relationship aims to share common information between features from same class and improves the quality of embeddings. 
Let the pair of speech segments $S_1 = [\: \boldsymbol{x^{(1)}_{1}, x^{(1)}_{2}, x^{(1)}_{3},...,x^{(1)}_{T_1}}\:]$ and $S_2 = [\: \boldsymbol{x^{(2)}_{1}, x^{(2)}_{2}, x^{(2)}_{3},...,x^{(2)}_{T_2}}\:]$ , the MSE loss becomes

\begin{equation} \label{MSE_Cor}
L_{mse}=\sum_{t=1}^{T_2} \| \boldsymbol{x^{(2)}_{t}} - D_{t}(E(S_1)) \| ^2    
\end{equation}
where $T_1$ and $T_2$ representing the segment length of $S_1$ and $S_2$ respectively. 
%Prior to the Cor-RAE training we use a pre-train standard RAE as weight initialization.  

\begin{figure}[t!]
  \setlength\belowcaptionskip{-0.8\baselineskip}
  \centering
  \includegraphics[width=0.95\linewidth]{RAE.jpeg}
  \caption{Siamese network architecture. Parameters are shared across the RAEs in Siamese network. The cosine distance is chosen as the similar metric for the acoustic phone embeddings.}
  \label{fig:RAE}
\end{figure}

    \subsection{Phone segment similarity for Siamese Network}
%To perform the mispronunciation detection using the acoustic embedding, 
In the phonological process of SSD speech, the realization of particular phoneme is different from the typical one, and the typical pronunciation is consistent across various context. 
Following this idea, we want the intra-class acoustic phone embeddings to be similar while the inter-class embeddings to be dissimilar. 
Given the label of each phone segment, we can form pairs of segments and adapt the Siamese network architecture to incoporate the idea of similarity evaluation in the SSD detection system. %we can form the phone pairs and model the Siamese network. 
In previous reserach works, Wang and Qin et al. \cite{wang2019child} used posterior features of phone attributes perform SSD detection of children speech via the Siamese network. The application of Siamese network in pronunciation evaluation of L2 speakers was also introduced by Wang and Zhang et al. \cite{8706597}.
The parameters of the RAEs in Siamese network are tied, as also in \cite{zhu2018siamese}. The embeddings are used to compute the Saimese loss and update the network parameters. 
Two loss functions of Siamese network are considered and compared in this work. The first one is the contrastive loss, denoted as $L_{c}$ It is expressed as:
%Loss_constrast
\begin{equation} \label{contrast_loss}
L_{c}=\dfrac{1}{2}y*d + \dfrac{1}{2}(1-y)*{max(0,m-d)}
\end{equation}
The contrastive loss function receives a pair of embeddings $\boldsymbol{z_{1},z_{2}}$ from the encoder outputs and its cosine distance $d$ is computed as the loss, where $d=1-cos(\boldsymbol{z_{1},z_{2}})$.
It aims to narrow the the cosine distance between the embeddings from the same class ($y=1$), and pull apart the distance if they are from different classes ($y=0$) and the computed distance exceeds the pre-defined margin $m$.

The second loss function introduced is the triplet loss, denoted as $L_{t}$. It takes three samples at each time, which includes an anchor, a positive and a negative. It is defined as: 
%Loss_triplet
\begin{equation} \label{triplet_loss}
L_{t}={max(0,m+d_{ap}-d_{an})}.
\end{equation}
where $d_{ap}$ and $d_{an}$ are the cosine distance of the anchor-positive pair and the anchor-negative pair respectively, and $d_{12}=0.5*(1-cos(\boldsymbol{z_{1},z_{2}}))$.

The final objective function of Siamese RAE combines the MSE and contrastive/triplet loss:
\begin{equation} \label{mse_contrast_loss}
\begin{split}
L_{mse,c}& = (1-w)*L_{c} +  w*\dfrac{L_{mse1}+Loss_{mse2}}{2}
\end{split}
\end{equation}
\begin{equation} \label{mse_triplet_loss}
\begin{split}
L_{mse,t} & = (1-w)*L_{t} +  w*\dfrac{L_{mse\_a}+L_{mse\_p}+L_{mse\_n}}{3}
\end{split}
\end{equation}
where $w$ is the scalar weight to balance the reconstruction loss and similarity loss. The Siamese network architecture can be referred to Figure \ref{fig:RAE}. %figure required


\begin{figure}[h]
  \setlength\belowcaptionskip{-0.8\baselineskip}
  \centering
  \includegraphics[width=\linewidth]{System_Diagram.jpeg}
  \caption{Speech sound disorder (SSD) detection system.} %The encoder was trained with the Siamese loss function. Each embedding of test speech segment is compared with the embeddings of the same class from the inventory.}
  \label{fig:system_design}
\end{figure}

\section{System Design} \label{sys}
%The pictorial illustration of the SSD detection system design is shown in Figure \ref{fig:system_design}. 
%After the model training, we preserve the encoder of the RAE to extract the phone level representations. 
%The embeddings of the training speech segments are first extracted and stored in the inventory. They refer to the standard articulation and they are used in the testing stage.
In clinical assessment of children's acquisition of consonants, each child is guided to pronounce a list of test words. The process is observed by the pathologists to decide if the child makes error in each pronunciation. %each consonant segment is correctly pronounced. 
This workflow is followed by our proposed SSD detection system, as illustrated in Figure \ref{fig:system_design}.
%The target consonant segment is first located and extracted by forced alignment. It is fed into the encoder to generate the fixed dimensional embedding.
The pronunciation evaluation is carried out by pairwise comparison between the embedding of test segment and all training segments from the same consonant. The training segments (in the top left of Figure \ref{fig:system_design}) are referred to standard pronunciations. All embeddings are extracted by the encoder, which is obtained from the trained RAE model.
The average cosine distance is computed from all data pairs. The binary decision is based on a pre-defined threshold. If the score is above the threshold, the test segment is classified as typical pronunciation. Else it is a disordered pronunciation. 
%In practice the detection system receives the audio of the target word. As in clinical session, the pathologists observes how the child articulates the consonant, the target consonant segment is first located and extracted. Phone alignment of the target word can be obtained by the child speech acoustic model. The acoustic features of the target segment is fed into the encoder. This outputs the compressed representation from the embedding layer. 
%The following pronunciation evaluation is implemented on the embedding level. Each embedding of test sample is compared to all embeddings of training samples of same category in pairwise sense, which gives an average cosine distance as the final score. A pre-defined threshold makes the binary decision. If the score is above the threshold, the test segment is classified as correct pronunciation. Otherwise it is considered as disordered pronunciation. 




\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Training\\ Data\end{tabular}}                  & \textbf{Type} & \textbf{Weight} & \textbf{EER(\%)} & \textbf{AUC}   \\ \hline
\multirow{3}{*}{\textbf{Child}}                                                   & \textbf{C}    & 0.2             & 12.381           & 0.929          \\ \cline{2-5} 
                                                                                  & \textbf{CV}   & 0               & 13.905           & 0.920          \\ \cline{2-5} 
                                                                                  & \textbf{C+CV} & 0.5             & 10.329           & 0.942          \\ \hline \hline
\multirow{3}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Child +\\ Adult\end{tabular}}} & \textbf{C}    & 0.3             & 10.794           & 0.941          \\ \cline{2-5} 
                                                                                  & \textbf{CV}   & 0               & 11.365           & 0.941          \\ \cline{2-5} 
                                                                                  & \textbf{C+CV} & \textbf{0.5}    & \textbf{9.206}   & \textbf{0.955} \\ \hline
\end{tabular}
\end{table}








% For example, a child of age four and a half is supposed to have mastered the affricate \textipa{/ts/}, but he is found to consistently substitute the phoneme \textipa{/ts/} by \textipa{/s/} .
% For instance, more than 90 percent of children should have acquired the affricate {/ts/} by the age of four and a half. \cite{to2013population}
%This symptom in which the desired phoneme, typically a consonant, being substituted by another consonant,



